Comparison of Various SLAM Systems for Mobile Robot in an Indoor Environment

This article presents a comparative analysis of a mobile robot trajectories computed by various ROS-based SLAM systems. For this reason we developed a prototype of a mobile robot with common sensors: 2D lidar, a monocular and ZED stereo cameras. Then we conducted experiments in a typical office environment and collected data from all sensors, running all tested SLAM systems based on the acquired dataset. We studied the following SLAM systems: (a) 2D lidar-based: GMapping, Hector SLAM, Cartographer; (b) monocular camera-based: Large Scale Direct monocular SLAM (LSD SLAM), ORB SLAM, Direct Sparse Odometry (DSO); and (c) stereo camera-based: ZEDfu, Real-Time Appearance-Based Mapping (RTAB map), ORB SLAM, Stereo Parallel Tracking and Mapping (S-PTAM). Since all SLAM methods were tested on the same dataset we compared results for different SLAM systems with appropriate metrics, demonstrating encouraging results for lidar-based Cartographer SLAM, Monocular ORB SLAM and Stereo RTAB Map methods.

==> Sections/implementation.tex <==
\section{Implementation}
\label{implementation}

\subsection{Lidar SLAM methods}
In this section, we discuss SLAM systems based on 2D lidar data. In ROS architecture we use \textit{urg\_node}, which produces \textit{sensor\_msgs/LaserScan message} that contains the array of ranging information. Each range information corresponds to the angle. We focused on popular systems and compare their performance in terms of map building and localization after two laps.

\subsubsection{GMapping}
GMapping was developed in 2007, and it is still the one of the most common systems for robot application. The system uses Particle filter and creates the grid-based map \cite{Grisetti2007}. The system subscribes to the \textit{sensor\_msgs/LaserScan message} and publishes  \textit{nav\_msgs/OccupancyGrid}, \textit{tf} transformation. The final map after two laps is presented in the Fig.  \ref{fig:SLAMmaps}\textit{(a)}. Different parameters of the system were tested. The final map does not represent the real map of the environment. The trajectory of the robot cannot be computed since there is no robust map of the environment. %This system cannot be used for this type of applications.

\subsubsection{Hector SLAM}
Hector SLAM system \cite{Kohlbrecher2011} was developed in 2011. The system subscribes to the \textit{sensor\_msgs/LaserScan message} and publishes  \textit{nav\_msgs/OccupancyGrid}, \textit{tf} transformation, and the pose with covariance message \textit{geometry\_msgs/PoseWithCovarianceStamped}. This information can be used for sensor fusion of systems based of Hector SLAM data. The system produces 2D map of environment precisely that can be used for navigation of mobile robot. The final map after two laps is presented in the Fig. \ref{fig:SLAMmaps}\textit{(b)}. 
The trajectory obtained from Hector SLAM system was compared with the marked line on the floor (which we refer as the ground truth), with conclusion of good fitting one to another. The trajectories are shown in the Fig. \ref{fig:SLAMmaps}\textit{(c)}. 
As far as the Hector SLAM path fits the ground truth, we make reasonable assumption that it produces the accurate measurements and can be used for trajectory validation of other SLAM systems.

\subsubsection{Cartographer}
Cartographer \cite{hess2016} system was developed in 2016. The system subscribes to the \textit{sensor\_msgs/LaserScan message} and publishes  \textit{nav\_msgs/OccupancyGrid}, \textit{tf} transformation.  The final map generated by this system after two UGV laps is presented in the Fig. \ref{fig:SLAMmaps}\textit{(d)}, and shows the best fitting from 2D Lidar maps to the real environment.
The trajectory obtained from Cartographer system was compared with the ground truth, and the Fig. \ref{fig:SLAMmaps}\textit{(e)} demonstrates the good result, which is relevant for indoor robotics applications. 

\subsubsection{Summary}
We tested three 2D Lidar SLAM systems: GMapping, Hector SLAM and Cartographer. The first system did not provide reliable results. The most important result in this section is comparison between Hector SLAM and Cartographer trajectories, which is presented in the Fig. \ref{fig:SLAMmaps}\textit{(f)}.
The trajectories fit perfectly. We use absolute trajectory error which is defined at the methodology section \ref{sec:metrics}. The results are presented in the Table \ref{tab:allTable}. The difference between two trajectories is less than 3 cm in RMSE, that allows to conclude that two systems produce actually the same results.

\begin{figure}[!htbp]
    \captionsetup{font=scriptsize}
    \centering
    \hfill
    \begin{subfigure}[b]{0.154\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/gmapping.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont GMapping map}
        \vspace{1mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.154\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/hector_map.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Hector SLAM map}
        \vspace{1mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.164\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/hector.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Hector SLAM path}
        \vspace{1mm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/cartographer.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Cartographer map}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.162\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/CartographerTraj.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Cartographer path}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.162\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/hectorCartographer.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Hector vs Cartographer}
        \vspace{0.5mm}
    \end{subfigure}
  \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Maps and UGV trajectories recovered from 2D Lidar SLAM methods.}
    \label{fig:SLAMmaps}
\end{figure}

\subsection{Monocular SLAM methods}
In this section, the results of ROS-based monocular SLAM systems are presented. All systems were tested on data from monocular Basler camera with the frame rate of about 20 fps. The processing of SLAM systems was provided by an external PC. The main disadvantage of these systems is scale ambiguity problem, which means that there is no information about the environment in an absolute scale. We use manual handling to solve this problem. 

\subsubsection{Parallel Tracking and Mapping (PTAM)}
PTAM is one of the keyframe-based visual SLAM system that allows to estimate 3D robot pose and build 3D map by tracking FAST features \cite{klein2007}. The system subscribes to the \textit{sensor\_msgs/Image} and publishes  \textit{geometry\_msgs/PoseWithCovarianceStamped}, \textit{tf} transformation. The system does not output a map to the ROS environment, therefore the map can be observed using the build-in tool. The feature detection and map visualization with camera pose estimation are presented in the Fig. \ref{fig:PTAM}\textit{(a-b)}.
We did not succeed to get reliable data from this system after two UGV laps. The system lost the track when robot had a turn, demonstrating a lack of robustness to lateral maneuvers. The process of map reinitialization after losing a track is presented in the Fig. \ref{fig:PTAM}\textit{(c)}.  

\begin{figure}[!htbp]
    \captionsetup{font=scriptsize}
    \centering
    \hfill
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/mptamc.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Feature detection}
        \vspace{1mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/mptamm.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Point cloud and path}
        \vspace{1mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/mptaml.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Reinitialization}
        \vspace{1mm}
    \end{subfigure}
  \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont  The UGV camera-based visualization with Monocular PTAM method.}
    \label{fig:PTAM}
\end{figure}

\subsubsection{Semi-direct Visual Odometry (SVO)}
SVO \cite{Forster2014} has a good integration with ROS, subscribes to the \textit{sensor\_msgs/Image} and publishes \textit{geometry\_msgs/PoseWithCovarianceStamped} for a robot pose, \textit{sensor\_msgs/PointCloud} for a map, and \textit{tf} for transformation. The process of feature detection and map with pose estimation are presented in the Fig. \ref{fig:SVO}. The system is not robust for this application since it loses track on robot turns, but can be used for additional information for straight UGV motion segments. 

\begin{figure}[!htbp]
    \captionsetup{font=scriptsize}
		\captionsetup[subfigure]{aboveskip=4pt,belowskip=0pt}
		\begin{subfigure}[b]{0.235\textwidth}
		    \captionsetup{font=scriptsize}
			\centering
		\includegraphics[width=\textwidth]{images/svoc.png} 
			\caption{\textnormal {\fontsize{8}{12}\fontfamily{ptm}\selectfont Feature detection}}
			\label{fig:robotmodel_a}
		\end{subfigure}
		\hfill
		\begin{subfigure}[b]{0.235\textwidth}
		    \captionsetup{font=scriptsize}
			\centering
		\includegraphics[width=\textwidth]{images/svom.png} 
			\caption{\textnormal {\fontsize{8}{12}\fontfamily{ptm}\selectfont Point cloud and trajectory}}
			\label{fig:robotmodel_b}
		\end{subfigure}
	\caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont The UGV camera-based visualization with Monocular SVO method.}
	\label{fig:SVO}
\end{figure}

\subsubsection{Dense Piecewise Parallel Tracking and Mapping (DPPTAM)}
DPPTAM is a direct system for pose estimation, which uses an assumption that regions with the same color belong to approximately the same plane \cite{Concha2015}. We can see the key point detection and plane fitting in the Fig. \ref{fig:DPPTAM}.
As far as the system lost tracking on robot turns, the system is not enough robust for this indoor application. 

\begin{figure}[!htbp]
    \captionsetup{font=scriptsize}
		\captionsetup[subfigure]{aboveskip=4pt,belowskip=0pt}
		\begin{subfigure}[b]{0.235\textwidth}
		    \captionsetup{font=scriptsize}
			\centering
		\includegraphics[width=\textwidth]{images/dpptam1.png}
			\caption{\textnormal {\fontsize{8}{12}\fontfamily{ptm}\selectfont Feature detection}}
			\label{fig:robotmodel_a}
		\end{subfigure}
		\hfill
		\begin{subfigure}[b]{0.235\textwidth}
		    \captionsetup{font=scriptsize}
			\centering
		\includegraphics[width=\textwidth]{images/dpptam2.png} 
			\caption{\textnormal {\fontsize{8}{12}\fontfamily{ptm}\selectfont Feature detection}}
			\label{fig:robotmodel_b}
		\end{subfigure}
	\caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont The UGV camera-based feature visualization with DPPTAM method.}
	\label{fig:DPPTAM}
\end{figure}

\subsubsection{Large Scale Direct monocular SLAM (LSD SLAM)}
LSD SLAM is the direct method, which uses a local image to image fitting, providing a pose prediction and building a dense map \cite{engel2014a}. LSD SLAM system has a loop closure option that gives an advantage for drift error compensation. The system has a poor ROS integration, subscribing to the \textit{sensor\_msgs/Image} and publishing \textit{tf} transformation. The process of key points detection and map with pose estimation are presented in the Fig. \ref{fig:MonoSLAM}\textit{(a,d)}.
After scale correction, the UGV trajectory was recovered and compared with Hector SLAM trajectory (the result is presented in the Fig. \ref{fig:MonoSLAM}\textit{(g)}). 
The computed metrics for trajectory evaluation is present in the Table \ref{tab:allTable}.
The system has a problem with a robot pose shift at the beginning of the map building since the map is not enough dense for precise localization. We can observe such a shift in the Fig. \ref{fig:MonoSLAM}\textit{(g)}. This shift can be filtered with a robot motion model. Thus, the system is robust and after absolute scale recovery can be used for robot pose estimation and map building.

\begin{figure}[!htbp]
    \captionsetup{font=scriptsize}
    \centering
    \hfill
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/lsdc.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont LSD features}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/orbc.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont ORB features}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/dsoc.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont DSO features}
        \vspace{0.5mm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/lsdm.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont LSD point cloud}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/orbm.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont ORB point cloud}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/dsom.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont DSO point cloud}
        \vspace{0.5mm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/lsdslam.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont LSD-based path}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/orbslam.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont ORB-based path}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/dsoslam.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont DSO-based path}
        \vspace{0.5mm}
    \end{subfigure}
  \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont The features \textit{(a-c)}, maps \textit{(d-f)} and UGV trajectories \textit{(g-f)} recovered from the following Monocular SLAM methods: LSD, ORB and DSO.}
    \label{fig:MonoSLAM}
\end{figure}

\subsubsection{ORB SLAM (mono)}
The ORB SLAM is a feature-based system, which tracks ORB features for robot pose estimation \cite{Mur-Artal2015}. It creates sparse point cloud as the map. The system has loop closure detection and widely used for indoor robotics application. The process of features detection and map with pose estimation are presented in the Fig. \ref{fig:MonoSLAM}\textit{(b,e)}. The system requires an additional development to be integrated in ROS. The camera trajectory can be evaluated with \textit{txt}-file only after dataset processing.
The map is the good approximation of test environment. The trajectory of the robot from ORB SLAM system in comparison with Hector SLAM is shown in the Fig. \ref{fig:MonoSLAM}\textit{(h)}. The pose estimation is provided only during keyframes, and the information about the camera location is more sparse.
The metrics for the trajectory evaluation is presented in the Table \ref{tab:allTable}. 
The ORB SLAM system is very robust and provides the good approximation of robot trajectory if the task of absolute scale recovery is solved.

\subsubsection{Direct Sparse Odometry (DSO)}
DSO is the fully direct method \cite{engel2018}. The system uses the wrapper for ROS integration and requires an additional development for real robotics implementation. The main advantage of this system is the dense map. The process of key points detection and map with robot trajectory are presented in the Fig. \ref{fig:MonoSLAM}\textit{(c,f)}.
DSO publishes robot pose as \textit{tf} transformation. The DSO-based UGV trajectory in comparison with Hector SLAM is presented in the Fig. \ref{fig:MonoSLAM}\textit{(i)}. The system used without a loop closure, therefore the robot pose drift was accumulated during the first lap and created doubled environment objects in the map when the robot did the second lap. It is also possible that calibration difficulties \cite{yang2018} could lead to additional errors in our experiments. 
The metrics for the trajectory evaluation is presented in the Table \ref{tab:allTable}. 
DSO creates the dense map and the system is robust in terms of pose tracking, but the lack of loop close makes this map noisy. The system improved with a loop closure detection will give more precise results at the condition of careful calibration.

\subsubsection{Summary}
Monocular SLAM systems provide the information about UGV localization and mapping. But since there is no absolute scaling, it is required additional modules for scale recovery. Thus, monocular systems can be used as the source of additional information for pose estimation and map building.

\subsection{Stereo SLAM methods}
The main advantages of stereo SLAM systems that they provide with absolute scale estimation. The systems were processed offline by an external PC, using the dataset collected from ZED Stereolabs camera with the data stream of about 10 fps.

\subsubsection{ZEDfu}
ZEDfu is the software solution with closed source code, which was provided by ZED camera developer to solve SLAM problem. The UGV trajectory is computed on-board, using GPU-accelerated code. The robot trajectory is presented in the Figure \ref{fig:RTABORBZEDfu}\textit{(g)}. 
The metrics for trajectory evaluation are presented in the Table \ref{tab:allTable}.
For our indoor experiment the method provided sufficiently large RMSE (almost two robot sizes). Thus, the system is robust in terms of robot pose tracking, but the trajectory is not accurate for such type of robot navigation.

\subsubsection{Real-Time Appearance-Based Mapping (RTAB map)}
RTAB map is the feature-based SLAM system \cite{Labbe2014}, which has a loop close detection and good integration with ROS. The feature extraction, map and robot trajectory after two laps are presented in the Fig. \ref{fig:RTABORBZEDfu}\textit{(a,c,e)}. The system sometimes has the problem with pose estimation when the robot moves closer to monotonous walls. But the Failure Recovery System is able to detect the failure and determine a robot pose properly.
The robot trajectory from RTAB map system is presented in the Fig. \ref{fig:RTABORBZEDfu}\textit{(e)}. It has a shift at the end of the first lap, but after a loop close detection it relocates the robot position.
The metrics for trajectory evaluation are presented in the Table \ref{tab:allTable}.
The system is robust and accurate. It solves localization problem with accuracy comparable with Lidar methods without additional manipulations that allows to use it for indoor robotics applications.

\begin{figure}[!htbp]
    \captionsetup{font=scriptsize}
    \centering
    \hfill
    \begin{subfigure}[b]{0.237\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/rtabc.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont RTAB map features}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.237\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/sordca.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont ORB features}
        \vspace{0.5mm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.237\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/rtabm.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont RTAB map point cloud}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.237\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/sordm.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont ORB point cloud}
        \vspace{0.5mm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/rtabmap.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont RTAB map path}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/orbslamstereo.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Stereo ORB path}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.158\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/zedfu.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont ZEDfu path}
        \vspace{0.5mm}
    \end{subfigure}
  \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont 
  The features \textit{(a,b)}, maps \textit{(c,d)} and UGV trajectories \textit{(e-g)} recovered from Stereo SLAM methods: RTAB map, Stereo ORB and ZEDfu.}
    \label{fig:RTABORBZEDfu}
\end{figure}

\begin{comment}
\begin{figure}[!htbp]
    \captionsetup{font=scriptsize}
    \centering
    \hfill
    \begin{subfigure}[b]{0.154\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/rtabc.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont RTAB features}
        \vspace{1mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.154\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/rtabm.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont RTAB point cloud}
        \vspace{1mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.164\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/rtabmap.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont RTAB map path}
        \vspace{1mm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/sordca.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont ORB features}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.162\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/sordm.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont ORB point cloud}
        \vspace{0.5mm}
    \end{subfigure}
    \begin{subfigure}[b]{0.162\textwidth}
        \captionsetup{font=scriptsize}
        \includegraphics[width=\textwidth]{images/orbslamstereo.png}
        \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont Stereo ORB path}
        \vspace{0.5mm}
    \end{subfigure}
  \caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont The features \textit{(a,d)}, maps \textit{(b,e)} and UGV trajectories \textit{(c,f)} recovered from the following Stereo SLAM methods: RTAB map and ORB.}
    \label{fig:RTABORB}
\end{figure}
\end{comment}

\subsubsection{ORB SLAM (stereo)}
ORB SLAM system has also the stereo mode \cite{Mur-Artal2015}, which provides absolute scaling in metres. The feature detection, mapping and UGV pose estimation are presented in the Fig. \ref{fig:RTABORBZEDfu}\textit{(b,d,f)}. The metrics for UGV trajectory evaluation re presented in the Table \ref{tab:allTable}.
The ORB SLAM with stereo camera provides accurate pose estimation and create sparse 3D map, allowing robust robot localization and pose tracking for indoor applications.

\subsubsection{Stereo Parallel Tracking and Mapping (S-PTAM)}
One of the most modern systems is feature-based S-PTAM \cite{Pire2017}, which has a framework for SLAM problem with a loop closure detection. It has also a possibility to choose any key point detector and feature descriptor available in OpenCV. The feature detection, mapping and UGV pose estimation are presented in the Fig. \ref{fig:SPTAM}.
The system was tested in two modes with loop closure and without, and compared with Hector SLAM-based trajectory in the Fig. \ref{fig:SPTAM}\textit{(c,d)}.
The metrics for trajectory evaluation are presented in the Table \ref{tab:allTable}.
The system is very flexible in terms of keypoint detection and selection of feature descriptors. It has loop closure option but it can demonstrate problems with the default "Bag of Words"-based place recognition dataset. It is required to create the Bag of Words for indoor office application and test loop closure. The system is robust in terms of pose tracking, and has the sparse map. But the localization accuracy can be not enough for robot navigation.


\begin{figure}[!htbp]
    \captionsetup{font=scriptsize}
		\captionsetup[subfigure]{aboveskip=4pt,belowskip=0pt}
		\begin{subfigure}[b]{0.237\textwidth}
		    \captionsetup{font=scriptsize}
			\centering
		\includegraphics[width=\textwidth]{images/sptamc.png}
			\caption{\textnormal {\fontsize{8}{12}\fontfamily{ptm}\selectfont Feature detection}}
			\label{fig:robotmodel_a}
			\vspace{1mm}
		\end{subfigure}
		\hfill
		\begin{subfigure}[b]{0.237\textwidth}
		    \captionsetup{font=scriptsize}
			\centering
		\includegraphics[width=\textwidth]{images/sptamm.png}
			\caption{\textnormal {\fontsize{8}{12}\fontfamily{ptm}\selectfont Point cloud and trajectory}}
			\label{fig:robotmodel_b}
			\vspace{1mm}
		\end{subfigure}
		\hfill
		\begin{subfigure}[b]{0.237\textwidth}
		    \captionsetup{font=scriptsize}
			\centering
		\includegraphics[width=\textwidth]{images/sptam.png}
			\caption{\textnormal {\fontsize{8}{12}\fontfamily{ptm}\selectfont Loop closure - off}}
			\label{fig:robotmodel_a}
		\end{subfigure}
		\hfill
		\begin{subfigure}[b]{0.237\textwidth}
		    \captionsetup{font=scriptsize}
			\centering
		\includegraphics[width=\textwidth]{images/sptam2.png}
			\caption{\textnormal {\fontsize{8}{12}\fontfamily{ptm}\selectfont Loop closure - on}}
			\label{fig:robotmodel_b}
		\end{subfigure}
	\caption{\fontsize{8}{12}\fontfamily{ptm}\selectfont The features \textit{(a)}, maps \textit{(b)} and UGV trajectories \textit{(c,d)} recovered from the following S-PTAM method.}
	\label{fig:SPTAM}
\end{figure}

\subsubsection{Summary}
Stereo visual SLAM systems provide metric information about UGV localization. The results for stereo systems: Real-Time Appearance-Based Mapping (RTAB map), ORB SLAM, Stereo Parallel Tracking and Mapping (S-PTAM) can be accurate enough at solving localization problems for indoor robotics applications. 
